Census Tract License Areas: Disincentive for Sharing the 3.5GHz band?

Flexible licensing model is a necessary enabler of the technical and procedural complexities of Spectrum Access System (SAS)-based sharing framework. The purpose of this study is to explore the effectiveness of 3.5GHz Licensing Framework - based on census tracts as area units, areas whose main characteristic is population. As such, the boundary of census tract does not follow the edge of wireless network coverage. We demonstrate why census tracts are not suitable for small cell networks licensing, by (1) gathering and analysing the official census data, (2) exploring the boundaries of census tracts which are in the shape of nonconvex polygons and (3) giving a measure of effectiveness of the licensing scheme through metrics of area loss and the number of people per census tract with access to spectrum. Results show that census tracts severely impact the effectiveness of the licensing framework since almost entire strategically important cities in the U.S. will not avail from spectrum use in 3.5GHz band. Our paper does not seek to challenge the core notion of geographic licensing concept, but seeks a corrective that addresses the way the license is issued for a certain area of operation. The effects that inappropriate size of the license has on spectrum assignments lead to spectrum being simply wasted in geography, time and frequency or not being assigned in a fair manner. The corrective is necessary since the main goal of promoting innovative sharing in 3.5 GHz band is to put spectrum to more efficient use.

==> Conclusions.tex <==
\section{Conclusions}
\label{sect:Conclusions}
The main conclusion from the detailed analysis of census tracts is that they do not provide a good basis on which to build a licensing framework. The FCC rightly recognizes that smaller license areas provide the potential for unlocking efficient sharing of spectrum in 3.5GHz band using small cell deployments. But as out results have shown, even under propagation conditions that are favorable, many unit license areas are rendered unusable and that potential is not unlocked.

%Towards the goal of enabling more efficient use with the sharing framework for 3.5GHz, FCC recognized the smaller license areas as a way to unlock the potential of efficient 3.5GHz sharing, favoring the small cell deployments in the band. However, the license area unit selected does not take into account the spectrum usage at all - the license area boundary is completely dependent on the demographics and the area size of the census tract. As a consequence, spectrum is being wasted over the area, as we have shown, and that fact puts the actions towards more efficient spectrum usage in a closed loop. This licensing model cannot sustain to support the necessary flexibility in the framework to enable sharing and effective coexistence of such diverse users in 3.5GHz.

The problem of spectrum waste over the license area, reflected through the percentage of area loss and number of people precluded from spectrum use points to the fact that the boundaries of census tracts are not appropriate boundaries for a license area in a geographic licensing scheme envisioned for 3.5 GHz band. Not only that they mismatch with the spectrum propagation of small cell deployments, the main deployments that  could put 3.5 GHz spectrum to more efficient use, but also finding the CBRS-allowed remains a problem with no solution even if the boundary limits are less stringent. In highly dense urban areas, census tracts are so small that it is not possible to form the CBRS-allowed area at all to fit the diverse spectrum usage so the interference between adjacent tracts is reduced. As we have shown, the smaller the census tracts are, more spectrum is wasted over the area.

Size of the license territory is one aspect of the license design. However, to design a flexible license based on geographic area, it is necessary to embed efficient interference protection mechanism in terms of limits on the license boundary, as well. 

Getting the licensing framework right is essential. The landscape in spectrum management has changed, in that it is accepted that some form of spectrum sharing will be part of the future. However it is still an open question as to which approaches will succeed. The 3.5GHz SAS-based sharing promises much and may be hampered in delivering if census tracts are at the core of its licensing framework. 

Therefore we propose the following geographic licensing models to take into consideration towards building an effective licensing framework that can fully support the SAS potential. Geographic area of deployment calculated based on the predicted actual spectrum usage should be the base area unit of the licensing scheme, i.e. area whose size is not fixed nor created for purposes other than spectrum usage. Describing the actual spectrum usage of an operator's network is a valid research question we plan to address in our future work, in order to investigate a particular challenge of how different network deployments need to be to be allocated in the same license area. 

%several SAS challenges: how different deployments would need to be to be allocated the same license area, if the rules are revised.
The model of spatial sharing that is adopted for the borders of the U.S and Canada and the U.S. and Mexico is an sharing arrangement in 800MHz band that is based on the geographic area so that the edge users on the borders can be served. 

We are pointing out that it is worth re-considering the licensing scheme, because the size and the shape of the license area matters. As we have shown, it affects the spectrum utilisation in different ways. To grant licenses that are geographically based in a meanigful way, license design needs to be based on these recommendations:(1) the license area should not be of fixed size, and (2) license should be issued based on actual spectrum use. 
%The problem of spectrum waste over the license area, reflected through the percentage of the area loss and population per area loss in Manhattan, Washington and San Francisco in our study, points to the following conclusions.

%Boundaries of census tracts which are created based on their population are not appropriate boundaries for a license area in a geographic licensing scheme envisioned for 3.5 GHz band. They mismatch with the spectrum propagation of small cell deployments, the main deployments that  could put 3.5 GHz spectrum to more efficient use.

%We explored census tracts through their main characteristics: population and area. We considered metrics of area loss and population per area loss as proxy of spectrum utilization.
%% Farely simple metrics of area loss and population per area loss provided us with an insight into potential spectrum waste under this licensing regime. 
%
%The huge variety of census tracts in terms of size and shape for the network operator will mean in terms of variety of conditions in the network, that the type of planning applied to one census tract does not hold for the other census tract, perhaps even adjacent one.

 
% If the license is issued for a census tract the percentage of loss is so significant that other way of issuing geographic licenses needs to be considered. 
 
% To issue the license in a more flexible way, we would traditionally think that it means to issue it for a larger area. However, that does not foster the competition in this band, which is one of the main goals of the proposal on sharing the 3.5GHz in a more innovative, flexible and dynamic way. If the areas are smaller, we have shown that the smaller the census tract areas are, the more spectrum is wasted over the area. We further note that even if the  boundary limit is reduced, there is still a problem of 'resizing' the census tracts to fit the diverse spectrum usage so the interference between adjacent tracts is reduced. In highly densed urban areas, census tracts are so small that they cannot be 'resized' at all to form the CBRS-allowed area of deployment.
 
% Size of the license territory is one aspect of the license design. However, to design a flexible license based on geographic area, it is necessary to embed efficient interference protection mechanism in terms of limits on the license boundary, as well. Geographic area of deployment calculated based on the predicted actual spectrum usage should be the base area unit of the licensing scheme, i.e. area whose size is not fixed nor created for purposes other than spectrum usage.
% 
% Based on the diversity of users that SAS needs to accommodate in the band and the proposed rules on licensing, the only way towards more efficient spectrum use in this band is to issue the license based on the actual spectrum use. Consequently, interference mechanism should be adapted to take into account the actual spectrum usage. PA and GAA users would report to SAS the exact locations of their operation, predicted amount of time of spectrum usage, the requested frequencies to serve the desired area and target customers, as well as the technical specifications of their CBRS devices. 
%
%
%
%%We are pointing out that it is worth re-considering the licensing scheme, because the size and the shape of the license area matters. License area should
%
%
%We are pointing out that it is worth re-considering the licensing scheme, because the size and the shape of the license area matters. As we have shown, it affects the spectrum utilisation in different ways. To grant licenses that are geographically based in a meanigful way, license design needs to be based on these recommendations:(1) the license area should not be of fixed size, and (2) license should be issued based on actual spectrum use. 

%It is worth noting also that maximum signal levels allowed for CBRS deployments should not be too weak to penetrate the walls and obstacles in typical indoor small cell deployments, since that will discourage investment and deployment.The success of CBRS operations will depend on the operators' ability to deploy usable networks, but we aimed to explore the conditions for PA networks under specific technical rules proposed by FCC for their operations within census tract license area.
%- Size of a license territory is one aspect of a license design, the other is interference protection. Need to design a license in order to make sure that interference protection is very efficient. This could open discussion in conclusions (we started it in Introduction.)

%- 
%
%- Percentage of area loss for Manhattan reduces the impact of the band on spectrum sharing.
%
%- Huge variety in terms of size, this is variety of conditions for a network, whatever goes for one census tract does not apply to other census tract.

%- To issue the license in a more flexible way, could imply that it means to issue it for a larger area - but that does not contribute to the competition and more efficient spectrum use.
% To go for smaller area, does not provide enough flexibility either as we showed in our results: the smaller area you go, the more spectrum is wasted over the area. 
%
%- How do we grant licenses that are geographically based in a meaningful way?






%Boundary issues become far
%
%more acute as license areas get smaller. This is because, as geographic areas increase, their
%
%boundaries grow linearly while the overall area increases far more quickly (for example, as the
%
%square of the radius of a circular area). Conversely, reducing the size of a geographic area
%
%results in a very significant decrease in overall area, with only a linear decrease in the
%
%corresponding boundary length. 


%However, since there is no universal spectrum sharing metric which will give the answers to all the issues adequately, depending on receiver and transmitter characteristics.
%Here I put my findings about the metric, if needed.
%From the area loss results, we can conclude that percentage of spectrum waste over the area (ALP) is higher (it is even 100 \%) for areas where census tracts are smaller. This is the very notion that census tracts are based on, they tend to be smaller in highly dense urban areas and their size increases in less urbanised and rural areas. Also, for the areas where census tracts are small, to satisfy the boundary constraint of sharing rules is a more challenging problem, than in the case of larger census tracts, because of the fact that the license boundary decreases linearly but the area within that boundary decreases faster.
%
%On a higher note, if we think about the estimated population growth for the next 5 years in Manhattan, Washington DC and San Francisco, the loss of spectrum over the area and the unavailability of spectrum for network capacity consumers within census tract boundaries could disable efficient sharing in 3.5GHz in these areas completely. Based on these results, it does not seem like census tract licensing areas, embedded in current licensing framework, will be able to sustain as the basis of licensing scheme, reducing the impact of 3.5GHz for sharing, significantly. And in particular, demand and supply principle on which SAS assignments are based on will be hard to satisfy. 
%
%From Fig.\ref{DCd1} and Fig.\ref{DCd2} we can visualize the variety of census tracts in terms of their shape and size. Their high irregularity will have an impact on the conditions in the network deployed, if such areas are adopted as license areas for CBRS deployments. The potential variety for network conditions, imposed by census tracts characteristics could increase uncertainty for the operators who plan to target certain customer profile or provide service on few specific locations. This would negatively affect the goal of fostering the competition in the band and opening it for a diverse use. 



